Momentum Auxiliary Network for Supervised Local Learning

Deep neural networks conventionally employ end-to-end backpropagation for their training process, which lacks biological credibility and triggers a locking dilemma during network parameter updates, leading to significant GPU memory use. Supervised local learning, which segments the network into multiple local blocks updated by independent auxiliary networks. However, these methods cannot replace end-to-end training due to lower accuracy, as gradients only propagate within their local block, creating a lack of information exchange between blocks. To address this issue and establish information transfer across blocks, we propose a Momentum Auxiliary Network (MAN) that establishes a dynamic interaction mechanism. The MAN leverages an exponential moving average (EMA) of the parameters from adjacent local blocks to enhance information flow. This auxiliary network, updated through EMA, helps bridge the informational gap between blocks. Nevertheless, we observe that directly applying EMA parameters has certain limitations due to feature discrepancies among local blocks. To overcome this, we introduce learnable biases, further boosting performance. We have validated our method on four image classification datasets (CIFAR-10, STL-10, SVHN, ImageNet), attaining superior performance and substantial memory savings. Notably, our method can reduce GPU memory usage by more than 45\% on the ImageNet dataset compared to end-to-end training, while achieving higher performance. The Momentum Auxiliary Network thus offers a new perspective for supervised local learning. Our code is available at: https://github.com/JunhaoSu0/MAN.

==> 01_intro.tex <==
\section{Introduction}
\label{sec:intro}

The domain of deep learning has predominantly been governed by end-to-end backpropagation \cite{2}, a fundamental strategy for training these complex models. This technique necessitates computationally demanding calculations for loss functions, succeeded by a series of reverse-sequenced gradient propagations through each layer, all aimed at optimizing neural network parameters \cite{20, 21,22}. However, this training modality is incongruous with the operational mechanics of biological neural networks. Knowledge acquisition in the human brain largely pivots on local signal transmission between synapses \cite{7,35,36}, circumventing the need for global signals. Furthermore, the end-to-end training methodology engenders a locking issue \cite{1} for network parameter updates. Here, the parameters of each layer must abide by the completion of the entire forward and backward propagation process before they can be updated. This situation contributes to complications such as diminished parallel efficiency and escalated GPU memory consumption \cite{16,18}, thereby hindering training efficiency.

A potential alternative to end-to-end (E2E) training is local learning \cite{1,11,12,13,14,15,27,28,43}, a methodology that has gained traction in recent years as a solution to the aforementioned issues. In particular, supervised local learning \cite{15,27,28} partitions the network into several gradient-isolated local blocks. Each gradient-isolated local block relies on its independent auxiliary network for optimization, guided by local objectives. Upon receiving its local error signal, each local block can immediately update its parameters, effectively alleviating the update locking problem inherent in E2E training and significantly enhancing parallel efficiency during training \cite{45,46}.
Simultaneously, as the training process only necessitates the storage of gradients for each local block's main network and its auxiliary network, and no longer requires global gradient information, the GPU memory usage during training is considerably less than in E2E training \cite{16,18}. This results in significant computational resource savings.

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{f1.pdf}
    \caption{Comparison of (a) end-to-end backpropagation, (b) supervised local learning, and (c) our proposed method. Unlike E2E, supervised local learning separates the network into K gradient-isolated local blocks. Our method enables information interaction by introducing the Momentum Auxiliary Network before the auxiliary network.}
    \label{Figure 1}
\end{figure*}

However, despite these advantages, a significant performance disparity persists between current supervised local learning methods and end-to-end (E2E) training. This discrepancy in accuracy becomes pronounced when the network is fractionated into numerous local blocks. Existing supervised local learning methods predominantly concentrate on auxiliary network design \cite{28} and local loss enhancement \cite{15,27} for improved performance. While these advancements can ameliorate the performance of supervised local learning to a certain degree, they fail to rectify its myopic view issue.
Owing to the absence of information interaction between local blocks, each local block prioritizes the optimization of its local objective, often overlooking the global objective. In this process, some information that could be beneficial to the global objective may inadvertently be discarded.

In this paper, we introduce a Momentum Auxiliary Network designed to foster information communication between local blocks, thereby mitigating the existing shortcomings in supervised local learning and significantly enhancing their performance. Our approach primarily leverages the structure of the first layer of the subsequent local block adjacent to each local block, inserting it between the main network and auxiliary network of each local block. Its parameters are updated using local gradients in conjunction with Exponential Moving Average methods \cite{34}. The efficacy of our method has been validated through a series of experiments conducted on four widely used image classification datasets: CIFAR-10 \cite{25}, STL-10 \cite{31}, SVHN \cite{30}, and ImageNet \cite{32}. In summary, our primary contributions to this research are as follows:

\begin{itemize}
\item Our proposed Momentum Auxiliary Network facilitates information interaction between local blocks, alleviates the short-sightedness issue, and through experimentation, we have verified that it can enable each local block to learn more information that is beneficial to the global objective.

\item Our proposed Momentum Auxiliary Network is a universal plug-and-play method. It can be combined with any supervised local learning method and significantly enhance their performance, with only a minimal increase in memory usage.

\item Our proposed Momentum Auxiliary Network has demonstrated its effectiveness through experiments on benchmark image classification datasets, achieving state-of-the-art performance. Notably, on the ImageNet \cite{32} dataset, it achieved better performance than E2E training with significantly less memory usage.

\end{itemize}





==> 03_method.tex <==
\section{Method}
\subsection{Motivation}
The superior performance of E2E training can be attributed to its holistic approach, where the entire network updates its parameters using a global error signal. It is thus unquestionable that the interaction of information between neural network layers plays a pivotal role in the model's performance. However, in traditional supervised local learning methods, the hidden layers within each local block are updated based upon their respective auxiliary networks, devoid of any global loss feedback from the top layers \cite{41,42}. Previous related work \cite{15,27,28} primarily focuses on short-term gains during the optimization of local layers, potentially overlooking critical features that could enhance performance in subsequent layers. If we can enable each gradient-isolated local block to access information from subsequent layers, thereby facilitating information exchange between them, we can address the shortsightedness observed in other methods within the supervised local learning domain.

To realize this objective, we conceptualized a universal information exchange module, the Momentum Auxiliary Network, a simple parallel structure. This module is strategically positioned between the main network and the auxiliary network of each gradient-isolated local block. The principal design intent of this module is to foster information exchange between the current local block and the subsequent block. In this manner, the current local block is emancipated from local optimization objectives, thereby learning more features beneficial to the global objective, which effectively addresses the shortsightedness issue. Notably, this only incurs a minor increase in memory usage.


\subsection{Momentum Auxiliary Network Design}
We assume a deep neural network $N_{\Theta}: \mathrm{X} \rightarrow \mathrm{Y}$, we can represent the forward process of network training using the input $x \in \mathrm{X}$ as follows:

\begin{equation}
N_{\Theta}(x)=c \circ n^k \circ n^{k-1} \circ \cdots \circ n^1(x)
\end{equation}

\noindent where $\circ$ represents the function of each local neural network block, and $c(\cdot)$ shows the fully connected layer used for the final classification. $n^k(\cdot)$ indicates the operational function at local block $k, 1 \leq k \leq K . \Theta=\left\{p^i\right\}_{i=1}^{K+1}$ stands for the trainable parameters of all local blocks.

When train the k-th local neural network block, the training process of other supervised local learning methods can represent the forward process as follows:
\begin{equation}
m_{\Theta}^k(x^k)=f^k \circ \Phi^k \circ n^k(x^k),(1 \leq k \leq K-1)
\end{equation}


\noindent where $m_{\Theta}^k(\cdot)$ stands for the k-th trainable local block of the deep neural network, $f^k(\cdot)$ means the classifier of the k-th local block, $\Phi^k(\cdot)$ expresses the auxiliary network of the k-th local block. By computing the local loss ${\mathcal L}_k \left( m^k(x^k),Y \right)$, we can update the parameters of $m^k$ through local backpropagation, where $Y$ represents the training labels, and $x^k=SG(n^{k-1}(x^{k-1}))$, $SG$ stands for the stop-gradient operator, which is used to prevent the propagation of gradients between adjacent local blocks. Figure \ref{Figure 1}(c) shows the overview of our method in detail. To enable the information of each gradient-isolated local block to interact with subsequent block, we have designed a parallel enhancement module named Momentum Auxiliary Network. Specifically, when training the k-th local block, we perform a deep copy of the first layer of the next local block twice: $\eta_k^{\prime}, \eta_k^{\prime \prime}=\operatorname{deepcopy}\left(n_1^{k+1}\right)$, where $n_1^{k+1}$ stands for the first layer of the (k+1)-th local block. $\eta_k^{\prime}$ is updated based on the backpropagation of the k-th local block, while $\eta_k^{\prime \prime}$ is updated using Exponential Moving Average (EMA) \cite{34} to facilitate information exchange with the (k+1)-th local block, it can be written as:

\begin{equation}
\Theta\left(\eta_k^{\prime}\right)=Backpropagation\left( {\mathcal L}_k \left( m_{\Theta}^k(x^k),Y \right) \right)
\end{equation}


\begin{equation}
\Theta\left(\eta_k^{\prime \prime}\right)=m \times \Theta\left(\eta_k^{\prime \prime}\right)+(1-m) \times \Theta\left(n_1^{k+1}\right)
\end{equation}


\noindent where $\Theta(\cdot)$ expresses the trainable parameters within the network, and $m$ indicates the hyperparameter $momentum$.

By parallelizing network layers with different parameter update strategies $\eta_k^{\prime}$ and $\eta_k^{\prime \prime}$, we obtain our Momentum Auxiliary Network:

\begin{equation}
\eta_k(x^k)=\eta_k^{\prime}(x^k)+\eta_k^{\prime \prime}(x^k)
\end{equation}

In this case, the forward process of the k-th local block can be rewritten as follows:

\begin{equation}
m_{\Theta}^k(x)=f^k \circ \Phi^k \circ \eta^k \circ n^k(x^k),(1 \leq k \leq K-1)
\end{equation}

\noindent which need to note is that the last local block $m^{K}$ does not necessitate an auxiliary network. It is directly linked to the final classifier, and its parameters are updated based on the global loss $\mathcal L \left( N(x),Y \right)$. Furthermore, auxiliary networks are not deployed during the testing process, and the forward process aligns with E2E.

In order to minimize both the output and local losses, the optimization objective for the entire training process of supervised local learning is as follows:
\begin{equation}
\min _{\Theta, \varphi} (\mathcal L\left(N_{\Theta}(x), y\right)+\sum_{k=1}^{K-1} \mathcal L^k\left(f^k\left(\Phi^k\left(\eta^k\left(n^k(x^k)\right)\right)\right), Y\right))
\end{equation}


\noindent where $\varphi=\left\{m_{\Theta}^1, m_{\Theta}^2, \cdots, m_{\Theta}^{K-1}\right\}$ is comprised of a collection of the learnable parameters from the first $\mathrm{K}-1$ local blocks.

The $\eta_k^{\prime}$ component takes advantage of the network structure of its subsequent layers but does not share gradients with them. Its primary function is to bolster the learning capacity of the hidden layers within each local block. In contrast, $\eta_k^{\prime \prime}$ facilitates communication between local blocks through EMA-based parameter updates. These two components fulfill complementary roles, the harmonious interplay between internal learning capacity and external communication significantly boosts the overall performance of the supervised local learning methods.







==> _constants.tex <==
\def\paperID{4383}
\def\confName{CVPR}
\def\confYear{2024}

\def\paperTitle{Paper Title}

\def\authorBlock{
    Author 1\thanks{Equal contribution} \qquad
    Author 2\footnotemark[1] \qquad
    Author 3 \\
    Institute \\
    {\tt\small \{email, addresses\}@inst.edu}
}

% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> _macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

\usepackage{graphicx}	
\usepackage{amsmath}	
\usepackage{amssymb}	
\usepackage{booktabs}
\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw,dvipsnames]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}


==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\frenchspacing


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

